Classicalization and Quantization of Tachyon-like Matter on (non)Archimedean Spaces

We consider a class of tachyon-like potentials, inspired by string theory, D-brane dynamics and cosmology in the context of classical and quantum mechanics. Motivated by the trans-Plankcian problem in the very early stage of cosmological evolution of the Universe, we consider the theoretical role of DBI-type tachyon scalar field, defined over the field of real as well as $p$-adic numbers, i.e. archemedean and nonarchimedean spaces. To simplify the equation of motion for the scalar field, canonical transformations are defined and engaged. The corresponding quantum propagators in the Feynman path integral approach on real and nonarchimedean spaces are calculated and discussed, as are possibilities for a quantum adelic generalization and its application.

==> rrp_mathdefs.tex <==
%\newcommand{\opL}{\mathfrak{L}}
%\newcommand{\opN}{\mathfrak{N}}

%elliptic Jacobi functions
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}

\newcommand{\ddiv}{\ensuremath{\mathop{\operator@font div}\nolimits}}
\newcommand{\grad}{\ensuremath{\mathop{\operator@font grad}\nolimits}}
\newcommand{\artanh}{\ensuremath{\mathop{\operator@font artanh}\nolimits}}
\newcommand{\sech}{\ensuremath{\mathop{\operator@font sech}\nolimits}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}

\let\op@format\mathfrak
%\let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%

